On the Importance of Environments in Human-Robot Coordination

When studying robots collaborating with humans, much of the focus has been on robot policies that coordinate fluently with human teammates in collaborative tasks. However, less emphasis has been placed on the effect of the environment on coordination behaviors. To thoroughly explore environments that result in diverse behaviors, we propose a framework for procedural generation of environments that are (1) stylistically similar to human-authored environments, (2) guaranteed to be solvable by the human-robot team, and (3) diverse with respect to coordination measures. We analyze the procedurally generated environments in the Overcooked benchmark domain via simulation and an online user study. Results show that the environments result in qualitatively different emerging behaviors and statistically significant differences in collaborative fluency metrics, even when the robot runs the same planning algorithm.

==> macros <==
%\usepackage[math]{kurier}
%\usepackage[sc]{mathpazo}                   
%\renewcommand{\sfdefault}{kurier}


%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{amsthm}
%\usepackage{amsbsy}
\usepackage{pgfgantt}
\usepackage{xcolor}
\usepackage{times}
\usepackage{soul}
\usepackage[utf8]{inputenc}
\usepackage[small, skip=5pt]{caption}
\setlength{\belowcaptionskip}{-10pt}
\usepackage{microtype}
\usepackage{graphicx}
\graphicspath{ {figures/} }
%\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{booktabs} % for professional tables
\usepackage{subfiles}
\usepackage{csquotes}
\usepackage{cite} % Compacts [1]--[4] citations and adds spaces
\usepackage[numbers]{natbib}
\usepackage{multicol}
\usepackage{latexsym} 
\usepackage{url}
\usepackage{lastpage}
%\usepackage{enumitem}
%\usepackage[sc]{mathpazo}
\usepackage{longtable}
\usepackage{array}
\usepackage{colortbl}
\usepackage{multirow}
%\usepackage{enumitem}

\usepackage{subcaption}


\linespread{1.05}         % Palatino needs more leading (space between lines)
%\usepackage{setspace}
%\usepackage[numbers,sort&compress,square]{natbib}


\usepackage{etaremune}
\usepackage{array}
%\setmainfont[Mapping=tex-text]{Gentium Basic}
%\usepackage{fullpage}
\usepackage[margin=1in]{geometry}


\definecolor{blue4}{HTML}{051A33}
\definecolor{blue3}{HTML}{153760}
\definecolor{blue2}{HTML}{275183}
\definecolor{blue1}{HTML}{3F689A}
\definecolor{ddorange}{HTML}{EE7600}


\definecolor{blue}{HTML}{0029A3}
%\definecolor{blue}{rgb}{0.015,0.015,.406}

\usepackage[
  bookmarks=false,
  pdfpagelabels=false,
  hyperfootnotes=false,
  hyperindex=false,
  colorlinks,urlcolor= blue,citecolor=blue,
]{hyperref}

\usepackage{pgfplots}


\usepackage{tikz}
\usepackage{tikzscale}
\usepackage{blindtext}
\usepackage{tikz-qtree}

\usetikzlibrary{shapes}
\usetikzlibrary{calc} 
\usepackage[compact]{titlesec}


\usepackage{titlesec}
\titlespacing{\paragraph}{%
  0pt}{%              left margin
  0.3\baselineskip}{% space before (vertical)
  1em}%               space after (horizontal)  
\titlespacing{\subparagraph}{%
  0pt}{%              left margin
  0pt}{% 			  space before (vertical)
  0.5em}%             space after (horizontal)
\titleformat{\subparagraph}[runin]{\bfseries \itshape}{\theparagraph}{}{}


\usepgfplotslibrary{fillbetween}	

\definecolor{cfblue}{rgb}{0.258824,0.258824,0.435294}
\definecolor{dblue}{rgb}{.098,.243,.424}
\definecolor{dorange}{rgb}{0.72, 0.506, 0.125}
\definecolor{llblue}{rgb}{.447,.643,.831}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\paren}[1]{\left({#1}\right)}
\newcommand{\brackets}[1]{\left[{#1}\right]}
\newcommand{\braces}[1]{\left\{{#1}\right\}}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\inner}[1]{ \left\langle {#1} \right\rangle }
\newcommand{\one}{\boldsymbol{1}}
\newcommand{\order}{O}
\newcommand{\prg}[1]{\noindent\textbf{#1. }} 

\newtheoremstyle{rqstyle}
{2pt}
{0pt}
{\itshape}
{}
{\bfseries}
{.}
{.5em}
{}

\theoremstyle{rqstyle}
\newtheorem{RQ}{RQ}
\newtheorem{Study}{Study}


\newcommand{\snnote}[1]{\normalsize{\color{orange}(Stefanos:\ #1)}}

\newcommand*\rot{\rotatebox{90}}

%\setlength{\columnsep}{1pt}%



